360$^\circ$ Reconstruction From a Single Image Using Space Carved Outpainting

We introduce POP3D, a novel framework that creates a full $360^\circ$-view 3D model from a single image. POP3D resolves two prominent issues that limit the single-view reconstruction. Firstly, POP3D offers substantial generalizability to arbitrary categories, a trait that previous methods struggle to achieve. Secondly, POP3D further improves reconstruction fidelity and naturalness, a crucial aspect that concurrent works fall short of. Our approach marries the strengths of four primary components: (1) a monocular depth and normal predictor that serves to predict crucial geometric cues, (2) a space carving method capable of demarcating the potentially unseen portions of the target object, (3) a generative model pre-trained on a large-scale image dataset that can complete unseen regions of the target, and (4) a neural implicit surface reconstruction method tailored in reconstructing objects using RGB images along with monocular geometric cues. The combination of these components enables POP3D to readily generalize across various in-the-wild images and generate state-of-the-art reconstructions, outperforming similar works by a significant margin. Project page: \url{http://cg.postech.ac.kr/research/POP3D}

==> figures/scene_settings.tex <==
\begin{figure}[t!]    
\begin{center}
\includegraphics[width=0.7\linewidth]{figures/scene_settings_v1.png}
\end{center}
\vspace{-4.0mm}
\caption{\textbf{Scene Settings.} We assume that the target 3D object lies within a cube of length $l$ and place our virtual camera $\phi$ on a sphere of radius $r$. We introduce specific values in \Sec{\ref{sub:framework_overview}}}
\label{fig:scene_settings}
\end{figure}


==> tables/geometry_cmp.tex <==
\begin{table*}[t!]
\centering
\caption{\textbf{Quantitative comparison of F-score and Chamfer Distance}. Our model model not only achieves the best embedding similarity but also achieves the best naturalness score. NL, RL, MCC, P-e, and SS3D stands for~\cite{neuralLift}, ~\cite{realfusion}, ~\cite{MCC}, ~\cite{pointe}, and ~\cite{ss3d} respectively.}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccccc|cccccc}

\Xhline{2\arrayrulewidth}  & \multicolumn{6}{c|}{F-Score $\uparrow$ } & \multicolumn{6}{c}{Chamfer Distance $\downarrow$ } \\
             & NL   & RL   & MCC  &P-e   & SS3D & Ours    & NL   & RL   & MCC  &P-e   & SS3D & Ours  \\ \hline \hline 
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
Obj          & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\\hline
Mean         & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00    & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  \\
 \Xhline{2\arrayrulewidth}
\end{tabular}
%}
\label{table:geometry_cmp}
\end{table*}

